Correcting Faulty Road Maps by Image Inpainting

As maintaining road networks is labor-intensive, many automatic road extraction approaches have been introduced to solve this real-world problem, fueled by the abundance of large-scale high-resolution satellite imagery and advances in computer vision. However, their performance is limited for fully automating the road map extraction in real-world services. Hence, many services employ the two-step human-in-the-loop system to post-process the extracted road maps: error localization and automatic mending for faulty road maps. Our paper exclusively focuses on the latter step, introducing a novel image inpainting approach for fixing road maps with complex road geometries without custom-made heuristics, yielding a method that is readily applicable to any road geometry extraction model. We demonstrate the effectiveness of our method on various real-world road geometries, such as straight and curvy roads, T-junctions, and intersections.

==> figures/diagram.tex <==
\begin{figure}[t] %%% t: top, b: bottom, h: here
\centering
\includegraphics[width=0.97\columnwidth]{figures/fig1.png}
\caption{
\fix{I promise that the figure will be improved!}
Illustration of our mathematical framework.
The probing task is defined as extracting how much label $Y$ information is present inside the $L$-th intermediate representation given the input $X$, i.e., the mutual information $I(X; Y)$.
The data processing inequality demands the information to be nonincreasing, whereas empirical linear probing results often exhibit the maximum peak in the middle layer.
We prove that the difference between the theoretical and empirical information amount comes from the discrepancy between the optimal probe $T^*$ and the learned linear probe $T_\theta$.
Also, its difference shows the linear separability of the representation space, which can be roughly understood as the level of usefulness of directly utilizing the representations.
}
\label{figs:diagram}
\end{figure}

==> images/architecture_table.tex <==
\begin{table}[ht]
\centering

\resizebox{0.99\linewidth}{!}{%
\begin{tabular}[t]{lccccc}
\hline
Type&Filter size&Stride&Dilation&Outputs\\
\hline
%input image&-&-&-&256 x 256 x 3\\
conv&5 × 5&1 × 1&-&64\\
\hline
conv&3 × 3&2 × 2&-&128\\
conv&3 × 3&1 × 1&-&128\\
\hline
conv&3 × 3&2 × 2&-&256\\
conv&3 × 3&1 × 1&-&256\\
conv&3 × 3&1 × 1&-&256\\
dilated conv&3 × 3&1 × 1&2&256\\
dilated conv&3 × 3&1 × 1&3&256\\
dilated conv&3 × 3&1 × 1&4&256\\
dilated conv&3 × 3&1 × 1&5&256\\
dilated conv&3 × 3&1 × 1&6&256\\
dilated conv&3 × 3&1 × 1&7&256\\
dilated conv&3 × 3&1 × 1&8&256\\
dilated conv&3 × 3&1 × 1&9&256\\
conv&3 × 3&1 × 1&-&256\\
conv&3 × 3&1 × 1&-&256\\
\hline
deconv&4 × 4&1/2 × 1/2&-&128\\
conv&3 × 3&1 × 1&-&128\\
\hline
deconv&4 × 4&1/2 × 1/2&-&64\\
conv&3 × 3&1 × 1&-&32\\
output&3 × 3&1 × 1&-&3\\
\hline
\end{tabular}
}

\caption{The generator network architecture of our model, GLCRC.}
\label{tab:architecture}
\end{table}%


==> images/network_architecture.tex <==
\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\textwidth]{images/images_03_method/extended_GLCIC_architecture.png}
  \vspace{-1em}
  \caption{Architecture of our road geometry inpainting model, GLCRC.}
  \label{fig:network_architecture}
\end{figure*}



==> images/segmentation_fallacy.tex <==
\begin{figure}[t]
  \centering
  \subfloat[Salt-like noise]{\includegraphics[width=0.41\textwidth]{images/fallacies/salt.png}}
  \subfloat[Pepper-like noise]{\includegraphics[width=0.41\textwidth]{images/fallacies/pepper.png}}\\
  \subfloat[Blurring]{\includegraphics[width=0.41\textwidth]{images/fallacies/blur.png}}
  \subfloat[Cropped out]{\includegraphics[width=0.41\textwidth]{images/fallacies/crop.png}}
  \vspace{5mm}
  \caption{
    Various common noises found in road segmentation model predictions.
    Leftmost is the satellite imagery, middle is the ground truth, and the rightmost is the prediction outputs.
  }
  \label{fig:segmentation_fallacy}
\end{figure}

==> images/sota_table.tex <==
\begin{table}[t]
\centering
\resizebox{0.95\linewidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule

\multicolumn{13}{c}{Straight Road}\\
\midrule
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{Salt} & \multicolumn{3}{c|}{Pepper} & \multicolumn{3}{c|}{Blur} & \multicolumn{3}{c}{Crop} \\
\cline{2-13}
& Cor. & Com. & Qua. & Cor. & Com. & Qua. & Cor. & Com. & Qua. & Cor. & Com. & Qua. \\
\midrule
\cite{bakhtiari2017semi} & & & & & & & & & & & & \\
\cite{wang2016new} & & & & & & & & & & & & \\
\cite{Liu2019MultiscaleRC, sujatha2015connected, singh2013automatic} & & & & & & & & & & & & \\
Ours & & & & & & & & & & 0.846 & 0.898 & 0.924 \\
\bottomrule

\multicolumn{13}{c}{Curvy Road}\\
\midrule
\cite{bakhtiari2017semi} & & & & & & & & & & & & \\
\cite{wang2016new} & & & & & & & & & & & & \\
\cite{Liu2019MultiscaleRC, sujatha2015connected, singh2013automatic} & & & & & & & & & & & & \\
Ours & & & & & & & & & & 0.779 & 0.455 & 0.928 \\
\bottomrule

\multicolumn{13}{c}{T Junction}\\
\midrule
\cite{bakhtiari2017semi} & & & & & & & & & & & & \\
\cite{wang2016new} & & & & & & & & & & & & \\
\cite{Liu2019MultiscaleRC, sujatha2015connected, singh2013automatic} & & & & & & & & & & & & \\
Ours & & & & & & & & & & 0.786 & 0.809 & 0.928 \\
\bottomrule

\multicolumn{13}{c}{Intersection}\\
\midrule
\cite{bakhtiari2017semi} & & & & & & & & & & & & \\
\cite{wang2016new} & & & & & & & & & & & & \\
\cite{Liu2019MultiscaleRC, sujatha2015connected, singh2013automatic} & & & & & & & & & & & & \\
Ours & & & & & & & & & & 0.826 & 0.886 & 0.894 \\
\bottomrule
\end{tabular}
}

\vspace{5mm}

\caption{Comparing post-processing methods on four road types with four noise types. Cor., Com., and Qua., denotes Correctness, Completeness, and Quality, respectively.}
\label{tab:sota}
\end{table}

==> images/synthetic_fallacy.tex <==
\begin{figure}[t]
  \centering
  \subfloat[Salt]{\includegraphics[width=0.24\textwidth]{images/noises/salt.png}}
  \subfloat[Pepper]{\includegraphics[width=0.24\textwidth]{images/noises/pepper.png}}
  \subfloat[Blur]{\includegraphics[width=0.24\textwidth]{images/noises/blur.png}}
  \subfloat[Crop]{\includegraphics[width=0.24\textwidth]{images/noises/crop.png}}

  \vspace{5mm}
  \caption{
    Synthetic noise types based on common segmentation model fallacies.
    For Blur and Crop noise, we indicate the location where the noise applied by a red circle.
  }
  \label{fig:synthetic_fallacy}
\end{figure}

==> images/wrong_road_extraction.tex <==

\begin{figure}
  \centering
 \subfloat[Missing road shape]{\includegraphics[width=0.99\columnwidth]{images/images_extracted_road/missing.png}}\\
  \subfloat[Missing and wrong road shape]{\includegraphics[width=0.99\columnwidth]{images/images_extracted_road/missing_complex_roads.png}}
%   \subfloat[Missing and noisy road shape (figure taken from \cite{extracted_road})]{\includegraphics[width=0.99\columnwidth]{images/images_extracted_road/extracted_road.png}}
  \caption{
    Labeling errors in road map dataset.
    Figures directly taken from \cite{MnihThesis}. (a) misses a road segment of the curvy winding road shape in the middle of road map image (b) misses road segments of unstructured winding road shapes on the left and right top area of map and presents the wrong road shapes on the straight roads by missing side roads. 
    % (a) presents a missing circular road segment in label image (right) from aerial image (left) \cite{MnihThesis}, (b) presents a missing road segment and missing one road in parallel roads (right) from aerial image (left), (c) presents a missing road and noisy road segments in extracted road image (right) from aerial image (left) \cite{extracted_road} by semantic segmentation 
  }
  \label{fig:missing_wrong_road_extraction}
\end{figure}


% https://www.emerald.com/insight/content/doi/10.1016/j.aci.2018.07.004/full/pdf?title=segmentation-based-traversing-agent-approach-for-road-width-extraction-from-satellite-images-using-volunteered-geographic-information

% \cite{extracted_road}
